Robust Ordinal VAE: Employing Noisy Pairwise Comparisons for Disentanglement

Recent work by Locatello et al. (2018) has shown that an inductive bias is required to disentangle factors of interest in Variational Autoencoder (VAE). Motivated by a real-world problem, we propose a setting where such bias is introduced by providing pairwise ordinal comparisons between instances, based on the desired factor to be disentangled. For example, a doctor compares pairs of patients based on the level of severity of their illnesses, and the desired factor is a quantitive level of the disease severity. In a real-world application, the pairwise comparisons are usually noisy. Our method, Robust Ordinal VAE (ROVAE), incorporates the noisy pairwise ordinal comparisons in the disentanglement task. We introduce non-negative random variables in ROVAE, such that it can automatically determine whether each pairwise ordinal comparison is trustworthy and ignore the noisy comparisons. Experimental results demonstrate that ROVAE outperforms existing methods and is more robust to noisy pairwise comparisons in both benchmark datasets and a real-world application.

==> fig/decoder.tex <==
\centering
\begin{tikzpicture}
    \tikzstyle{main} = [circle, minimum size = 18mm, thick, draw = black!100, node distance = 16mm]
    \tikzstyle{dot} = [circle, draw = black!100, fill = black!100, inner sep = 0mm, minimum size = 2mm,
                        node distance = 16mm]
    \tikzstyle{factor} = [box, draw = black!100, fill = black!100, inner sep = 0mm, minimum size = 2mm,
                        node distance = 16mm]
    \tikzstyle{connect} = [-latex, thick]
    \tikzstyle{no_arrow} = [-, thick]
    \tikzstyle{box} = [rectangle, draw=black!100, thick]

    \node[main]     (r_i)         []                                              {\LARGE $\mathbf{v}_i$};
    
    \node[main]		(t_i)		[below = of r_i]
{\LARGE $ u_i $};    

    \node[main]     (x_i)       [right = of r_i, xshift = 0mm, yshift = -16mm, fill = black!30] {\LARGE ${\mathbf{x}}_i$};


    \node[main]     (r_j)     [below = of t_i]
     {\LARGE $ \mathbf{v}_j $};
    
    \node[main]		(t_j)		[below = of r_j]
{\LARGE $ u_j $};    

    \node[main]     (x_j)       [right = of r_j, xshift = 0mm, yshift = -16mm, fill = black!30] {\LARGE $\mathbf{x}_j$};


    \node[main]     (y_ij)       [left = of r_j, xshift = -10mm, yshift = 0mm, fill = black!30] {\LARGE $y_{ij}$};
    
    \node[main]     (w_ij)       [left = of t_i, xshift = -10mm, yshift = 0mm] {\LARGE $w_{ij}$};



    \node[dot]      (alpha)     [above = of w_ij,
    xshift =-16mm, yshift = 10mm, label = left:\LARGE $ \mu_w $]
    {};

    \node[dot]      (beta)     [above = of w_ij,
    xshift = 16mm, yshift = 10mm, label = left:\LARGE $ \sigma_w^2 $]
    {};


    \node[box, inner sep=3mm, fit= (t_i) (r_i) (x_i),
                xshift = 0mm, yshift = -1mm] (N_i) {};
    \node[text width = 15mm, right = of N_i, xshift = -20mm, yshift = -23mm]      {\LARGE $N$};

    \node[box, inner sep=3mm, fit= (t_j) (r_j) (x_j),
                xshift = 0mm, yshift = -1mm] (N_j) {};
    \node[text width = 15mm, right = of N_j, xshift = -20mm, yshift = -23mm]      {\LARGE $N$};

    \node[box, inner sep=5mm, fit= (y_ij) (w_ij),
                xshift = 2mm, yshift = -2mm] (N_ij) {};
    \node[text width = 30mm, right = of N_ij, xshift = -32mm, yshift = -28mm]      {\Large $(i,j) \in \mathcal{J}$};



    \path           (t_i)         edge        [connect]      (x_i)
				    (r_i)         edge        [connect]      (x_i)
				    (t_j)         edge        [connect]      (x_j)
				    (r_j)         edge        [connect]      (x_j)
				    (t_i)         edge        [connect]      (y_ij)
				    (t_j)         edge        [connect]      (y_ij)
				    (w_ij)        edge        [connect]      (y_ij)
				    (alpha)       edge        [connect]      (w_ij)
				    (beta)        edge        [connect]      (w_ij)
    ;
\end{tikzpicture}






==> fig/encoder.tex <==
\centering
\begin{tikzpicture}
    \tikzstyle{main} = [circle, minimum size = 18mm, thick, draw = black!100, node distance = 16mm]
    \tikzstyle{dot} = [circle, draw = black!100, fill = black!100, inner sep = 0mm, minimum size = 2mm,
                        node distance = 16mm]
    \tikzstyle{factor} = [box, draw = black!100, fill = black!100, inner sep = 0mm, minimum size = 2mm,
                        node distance = 16mm]
    \tikzstyle{connect} = [-latex, thick]
    \tikzstyle{no_arrow} = [-, thick]
    \tikzstyle{box} = [rectangle, draw=black!100, thick]

    \node[main]     (x_i)         [fill = black!30]             
    {\LARGE $\mathbf{x}_i$};
    
    \node[main]     (u_i)         [right = of x_i, yshift = -16mm]              
    {\LARGE $u_i$} ;
    
    \node[main]     (v_i)         [right = of x_i, yshift = 16mm]              
    {\LARGE ${\mathbf{v}}_i$} ;
    
    \node[main]     (x_j)         [below = of x_i, fill = black!30, yshift = -24mm]
    {\LARGE $\mathbf{x}_j$};
    
    \node[main]     (u_j)         [right = of x_j, yshift = -16mm]
    {\LARGE $u_j$} ;
        
    \node[main]     (v_j)         [right = of x_j, yshift = 16mm]
    {\LARGE ${\mathbf{v}}_j$} ;
    
    \node[main]     (w_ij)       [left = of x_i, yshift = -32mm, xshift = -5mm]
    {\LARGE ${w}_{ij}$} ;


    \node[box, inner sep=3mm, fit= (x_i) (u_i) (v_i),
                xshift = 0mm, yshift = -1mm] (N_i) {};
    \node[text width = 15mm, right = of N_i, xshift = -18mm, yshift = -25mm]      {\LARGE $N$};

    \node[box, inner sep=3mm, fit= (x_j) (u_j) (v_j),
                xshift = 0mm, yshift = -1mm] (N_j) {};
    \node[text width = 15mm, right = of N_j, xshift = -18mm, yshift = -25mm]      {\LARGE $N$};

    \node[box, inner sep=4mm, fit= (w_ij),
                xshift = 0mm, yshift = -2mm] (N_ij) {};
    \node[text width = 30mm, right = of N_ij, xshift = -30mm, yshift = -9mm]      {\LARGE $N \times N$};


    \path           (x_i)         edge        [connect]      (u_i)
                    (x_i)         edge        [connect]      (v_i)
                    (x_j)         edge        [connect]      (u_j)
                    (x_j)         edge        [connect]      (v_j)
                    (x_i)         edge        [connect]      (w_ij)
                    (x_j)         edge        [connect]      (w_ij)
    ;
\end{tikzpicture}






==> sections/abstract_v1.tex <==
% !TEX root = ../main.tex
In recent years, disentanglement learning methods under  Variational Autoencoder (VAE) framework have gained substantial popularity. However, without introducing supervision, it is not guaranteed that the factor of interest can be successfully recovered~\citep{locatello2018challenging}. Motivated by a real-world problem, we propose a setting where the user provides pairwise ordinal comparisons between instances based on a factor to be disentangled. Since the pairwise comparisons are usually noisy, we propose a new method we call Robust Ordinal VAE (ROVAE) to learn disentanglement of latent variables of interest by making use of the observed noisy pairwise ordinal labels. We introduce a non-negative random variable in the model, such that ROVAE can automatically determine whether each pairwise ordinal label is trustworthy, and ignore noisy ordinal labels. Experimental results demonstrate that ROVAE outperforms existing methods and is more robust to noisy labels in both benchmark datasets and a real-world application.

==> sections/experiment_v1.tex <==
% !TEX root = ../main.tex

\section{Experiments}
\label{sec:Experiments}

In this section, we evaluate our method by performing experiments on both benchmark and real-world dataset. In the following, we first introduce the competitive method and the quantitative metrics used in this paper. Then, we introduce the performance of our method when noisy labels are observed in the benchmark datasets. Later, we present the results where we apply our method to analyze the real-world COPD dataset. Finally, we present some results of ablation study.

\subsection{ Competitive Method and Quantitative Metrics }

To demonstrate that ROVAE is more robust to the noise, we compare it with a Vannilla Ordinal VAE (VOVAE). VOVAE shares a similar framework of ROVAE, but fixes $s_{ij} = 1$.
We also compare ROVAE with existing unsupervised disentanglement approaches, including $\beta$-VAE, HCV, factor VAE, $\beta$-TCVAE. We have introduced these methods in Section \ref{sec:background_VAE}. 

In order to measure the performance quantitatively, we compare the methods based on two criteria: Mutual Information Gap (MIG) and regression/classification error. 

MIG is a popular measure for unsupervised disentanglement, first introduced by \cite{chen2018isolating}. Since we introduce supervision in our model, we use a variant of it, defined as
\begin{equation}
    \label{equ:MIG}
    MIG = \frac{1}{ \mathcal{H}(t) } \left( \mathcal{I} (u; t) - \max_{d \in \{1 \ldots D \}} \mathcal{I} (v_d; t) \right),
\end{equation}
where $u$ and $\mathbf{v}$ represent latent variables that represent latent variables that are relevant and irrelevant to the factor of interest, respectively, as introduced in Section \ref{sec:method_framework} and $t$ denote the ground-truth factor of variations of interest. We let $\mathcal{I}(\cdot;\cdot)$ denote the mutual information between two random variables, and $\mathcal{H}(\cdot)$ be the entropy of a random variable. Both $\mathcal{I}(\cdot;\cdot)$ and $\mathcal{H}(\cdot)$ can be estimated empirically, as explained by \citet{chen2018isolating}. 
MIG in Equation (\ref{equ:MIG}) is defined based on the intuition that we want $u$ to be related to $t$ but each $v_d$ to be independent of $t$. Note that MIG in Equation (\ref{equ:MIG}) can be negative because $\mathcal{I}(u;t)$ might be smaller than $\mathcal{I}(v_d;t)$ with a certain $d \in \{1, \ldots, D\}$, especially when we introduce noise to the labels.

In addition to MIG, we also want to investigate how well $u$ predicts $t$. Therefore, we train a $5$ Nearest Neighbour (5-NN) regressor/classifier that predicts $t$ using $u$. We report the r-squared value ($r^2$) for real-value $t$, we report Cohen's kappa ($\kappa$) for discrete $t$. Both $r^2$ and $\kappa$ have a maximum value of $1$ represent a better prediction, and a higher value indicates a better performance.

In the experiments, we also compute the quantitative measures for unsupervised disentanglement methods, where $u$ and $\mathbf{v}$ are not defined. For these variables, we pick the dimension of latent variable that has the maximum mutual information with respective to the ground-truth $t$ in the training set as $u$. The remaining latent variables are regarded as $\mathbf{v}$ in the computation.
\subsection{ Benchmark Datasets }

We evaluate our methods on four datasets:  Yale Faces~\citep{georghiades2001few}, 3D chairs~ \citep{aubry2014seeing} and 3D cars \citep{krause20133d} and UTKFace \citep{zhifei2017cvpr}. The details of these datasets are summarized in Table~\ref{tbl:dataset}. For each dataset, we generate a subset of pairwise ordinal labels based on comparing the ground-truth factor of variations, as shown in the table. Unless specified otherwise, we let the number of observed pairwise labels be $5,000$. Note that for 3D chairs and 3D cars datasets, we only include the instances with azimuth rotations between $0$ to $180$ degrees. We do not include the remaining instances because azimuth is cyclic. The ordinal comparison between two azimuth values might be unclear if we include all instances.

We want to measure the robustness of the proposed ROVAE against noisy ordinal labels. We consider the noise of two types:
(1) We first generate the pairwise ordinal labels by observing whether the ground-truth factors satisfying $t_1 \le t_2$. Then we flip the generated labels with probability $0 \le \eta \le 0.5$. Note that we do not consider the case when $\eta>0$, because it is equivalent to pairwise labels $t_1 > t_2$ with $1 - \eta$ flipped labels. This type of noise simulates that the user makes mistakes in labelling.
(2) We first generate random Gaussian noise $ \epsilon_1,\epsilon_2 \sim \mathcal{N}(0, \sigma^2)$. Then we generate the pairwise ordinal labels by observing whether $\tilde{t}_1+\epsilon_1< \tilde{t}_2 +\epsilon_2$ is true or not, where $\tilde{t}_1$ and $\tilde{t}_2$ are the normalized ground-truth factor of variations with zero mean and unit variance. This type of noise simulates that the user is more likely to make mistakes if two instances are similar with each other in terms of $t$. 

\subsubsection{Quantitative Comparisons}
We plot the MIG and $r^2$ after introducing the two types of noise in Figure \ref{fig:noise_eta} and \ref{fig:noise_sigma}, respectively. We observe in the figures that when the noise level is low, ROVAE does not always outperform VOVAE. However, when the noise level is moderate, ROVAE gives a higher $r^2$ and MIG than VOVAE consistently. When we further increase the noise level, both methods fail. By comparing the performance of ROVAE and VOVAE, we conclude that after introducing the trustworthiness score, ROVAE is able to generate more robust results.

In Figure \ref{fig:noise_eta} and \ref{fig:noise_sigma}, we performance of the unsupervised learning methods are plotted with a horizontal line. These methods do not make use of the labels, and therefore are not affected by the noisy labels. We observe that ROVAE and VOVAE outperform the unsupervised methods when the noise level is low or moderate. The results show that introducing pairwise ordinal labels is helpful in the disentangling tasks, and it is unlikely to disentangle the factor of interest if we do not introduce any supervisions.

\subsubsection{Qualitative Comparisons}
To compare the methods qualitatively when noisy pairwise label is presented, we generate some plots for the 3D chairs dataset, where $20\%$ of the labels are flipped ($\eta = .2$) as an example. We include the $\beta$VAE in addition to ROVAE and VOVAE, because it is the best unsupervised method for this dataset. 


To visualize whether or not the methods embed the instances based on the factor of interest, we plot some embedding results for the instances in the test set in Figure \ref{fig:embedding_ROVAE}, \ref{fig:embedding_VOVAE} and \ref{fig:embedding_betaVAE}. In the plots, we use different colors to represent instances with different ground-truth values. As shown in Figure \ref{fig:embedding_ROVAE}, the latent representation $u$ generated by ROVAE is consistent with the ground-truth factors, although a moderate level of noise is presented. In contrast, VOVAE is more affected by the noise introduced, as shown in Figure \ref{fig:embedding_VOVAE}. We observe more overlapping of dots with different colors. Although $\beta$VAE is not affected by the noise, it does not give good embedding, as shown in Figure \ref{fig:embedding_betaVAE}. Without introducing supervision, it is not guaranteed that unsupervised methods can recover the ground-truth factor of variations. By comparing Figure \ref{fig:embedding_ROVAE}, \ref{fig:embedding_VOVAE} and \ref{fig:embedding_betaVAE}, we conclude that the embedding results of ROVAE are more consistent with the ground-truth factor of interest in this task.


To illustrate whether or not the models disentangle the factor of interest and represent it with the latent representation $u$, we encode the instances into $[u, \mathbf{v}]$, keep $\mathbf{v}$ constant but manipulate $u$ and then generate images by decoding the results. We include some results in Figure \ref{fig:generated_ROVAE}, \ref{fig:generated_VOVAE} and \ref{fig:generated_betaVAE}. In Figure \ref{fig:generated_ROVAE}, we observe that the chairs generated by ROVAE rotate when we change the values of $u$. However, due to the introduced noise, the chairs generated by VOVAE do not rotate as much, as shown in \ref{fig:generated_VOVAE}. We can also observe rotation of generated chairs in Figure \ref{fig:generated_betaVAE}, indicating $beta$VAE is able to disentangle the factor of intrest without supvervision. However, the results are not as good as those generated by ROVAE. By comparing Figure \ref{fig:generated_ROVAE}, \ref{fig:generated_VOVAE} and \ref{fig:generated_betaVAE}, we conclude that ROVAE is a better approach to disentangle the factor of interest when noisy ordinal labels are presented.



\begin{figure}
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[height=1\textwidth, trim={0cm 1cm 1cm 2cm}, clip]
        {fig/chairs_embedding_ROVAE.png}
        \caption{Embedding results of ROVAE.}
        \label{fig:embedding_ROVAE}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[width=1\textwidth]{fig/chairs_recon_ROVAE.png}
        \caption{Generated images of ROVAE by manipulating $u$.}
        \label{fig:generated_ROVAE}
    \end{subfigure}    
    \\
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[height=1\textwidth, trim={0cm 1cm 1cm 2cm}, clip]
        {fig/chairs_embedding_VOVAE.png}
        \caption{Embedding results of VOVAE.}
        \label{fig:embedding_VOVAE}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[width=1\textwidth]{fig/chairs_recon_VOVAE.png}
        \caption{Generated images of VOVAE by manipulating $u$.}
        \label{fig:generated_VOVAE}
    \end{subfigure}        
    \\
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[height=1.\textwidth, trim={0cm 1cm 1cm 2cm}, clip]
        {fig/chairs_embedding_betaVAE.png}
        \caption{Embedding results of $\beta$VAE.}
        \label{fig:embedding_betaVAE}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.47\columnwidth}
        \includegraphics[width=1\textwidth]{fig/chairs_recon_betaVAE.png}
        \caption{Generated images of $\beta$VAE by manipulating $u$.}
        \label{fig:generated_betaVAE}
    \end{subfigure}   
    \caption{Embedding and reconstruction results for the 3D chairs dataset, where $20\%$ of the labels are flipped ($\eta = .2$).}
\end{figure}



\begin{table*}[t]
\caption{The Benchmark Dataset}
\label{tbl:dataset}
\centering
\begin{adjustbox}{width=1.\textwidth, center}  
  \begin{tabular}{lcccl}
    \toprule
    Dataset   & Training instances & Held-out instances & Image size & The ground-truth factor \\
    \midrule
    Yale Faces & $1,903$ & $513$& $64 \times 64 \times 1$ & Lighting Angles
    \\
    3D chairs & $69,131$ & $17,237$ & $64 \times 64 \times 3$ & Azimuth Rotations ( $0$\textemdash$180 ^{\circ} $ )
    \\
    3D cars & $14,016$ & $3,552$ & $128 \times 128 \times 3$ & Azimuth Rotations  ( $0$\textemdash$180 ^{\circ} $ )
    \\
    UTKFace & $37,932$ & $9,484$ & $200 \times 200 \times 3$ & Ages
    \\
    \bottomrule
  \end{tabular}
\end{adjustbox}  
\end{table*}


\begin{figure*}[t]
\begin{minipage}{.9\textwidth}
    \centering
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_chairs_.png}
        \caption{$r^2$ for the chairs dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_cars_.png}
        \caption{$r^2$ for the cars dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_Yale_.png}
        \caption{$r^2$ for the Yale dataset.}
    \end{subfigure}    
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_UTK_.png}
        \caption{$r^2$ for the UTKFace dataset.}
    \end{subfigure}    
    \\
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_chairs_.png}
        \caption{MIG for the chairs dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_cars_.png}
        \caption{MIG for the cars dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_Yale_.png}
        \caption{$r^2$ for the Yale dataset.}
    \end{subfigure}
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_UTK_.png}
        \caption{$r^2$ for the UTKFace dataset.}
    \end{subfigure}
    \caption{Plots of $r^2$ and MIG against different noise level $\eta$, where we randomly flip the ground-truth pairwise ordinal labels with probability $\eta$. }
    \label{fig:noise_eta}
\end{minipage}
\begin{minipage}{.9\textwidth}
    \centering
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_chairs.png}
        \caption{$r^2$ for the chairs dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_cars.png}
        \caption{$r^2$ for the cars dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_Yale.png}
        \caption{$r^2$ for the Yale dataset.}
    \end{subfigure}    
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/r2_UTK.png}
        \caption{$r^2$ for the UTKFace dataset.}
    \end{subfigure}    
    \\
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_chairs.png}
        \caption{MIG for the chairs dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_cars.png}
        \caption{MIG for the cars dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_Yale.png}
        \caption{MIG for the Yale dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
        \includegraphics[width=1\textwidth]{fig/MIG_UTK.png}
        \caption{MIG for the UTKFace dataset.}
    \end{subfigure}
    \caption{Plots of $r^2$ and MIG against the noise level $\sigma^2$, where we apply a Gaussian noise with variance $\sigma^2$ to the ground-truth factors before we generate labels based on the pairwise comparison.}
    \label{fig:noise_sigma}
    \end{minipage}
    \end{figure*}






\subsection{ The COPD Dataset }

A real-world application of ROVAE is to learn the factor of disease severity based on CT images in the COPD dataset (with over 9K patients), where we generate pairwise ordinal labels based on the GOLD criteria. As discussed in Section \ref{sec:introduction},  we consider these labels noisy. 

In addition of the GOLD criteria, we also train 5-NN model using the learned latent variable $u$ to predict other two measures for disease severity including (1) \texttt{Emphesyma\%} that measures the percentage of destructed lung tissue and (2) \texttt{GasTrap\%} that amounts gas trapped in lung. We report $\kappa$ and $r^2$ measured for the held-out data in Table \ref{tbl:COPD}. We observe that ROVAE outperforms VOVAE and all unsupervised methods in terms of predicting these measurements. In the table, we also include the prediction performance using the GOLD criteria. We observe that the severity variable learned by ROVAE gives better prediction for Emphesyma\% and GasTrap\% compred with the GOLD criteria. This suggests that ROVAE does not simply learn a latent representation that predicts the GOLD criteria as accurately as possible. By ignoring a subset of noisy ordinal labels, ROVAE might be able to discover a better measurement for disease severity based on the CT image.

We visualize the learned disease severity measurement by manipulating $\mu$ in Figure \ref{fig:lung}. We observe in the figure that with increased $u$, the reconstructed image tend to have a smaller heart size in comparison to the lungs and diaphragms tend to be more flattened, indicating a more severe COPD disease. The figure illustrates that ROVAE is able to disentangles the disease severity in the CT images.

\begin{table*}[t]
    \centering
    \caption{Results on the COPD Dataset}
    \label{tbl:COPD}
    \begin{tabular}{l l c c c c c c c}
    \toprule
     & & ROVAE & VOVAE & $\beta$VAE & HCV & Factor VAE & $\beta$TCVAE & GOLD criteria
    \\
    \midrule
    $\kappa$ & GOLD criteria
    & $.663$ & $.542$ & $.149$ & $.154$ & $.241$ & $.165$ & $\mathbf{1.00}$
    \\
    \midrule
    \multirow{2}{*}{$r^2$}  & \% Emphasema
    & $\mathbf{.491}$ & $.322$ & $-.215$ & $-.070$ & $-.226$ & $.047$ & $.244$
    \\
    & \% Gas Trapped
    & $\mathbf{.558}$ & $.401$ & $-.159$ & $-.089$ & $-.249$ & $.123$ & $.398$
    \\
    \bottomrule
    \end{tabular}
    
    \label{tab:my_label}
\end{table*}


\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{fig/posterior.png}
    \caption{The aggregated posterior distribution $q(w)$.}
    \label{fig:lung}    
\end{figure}

\begin{figure}[t]
    \begin{subfigure}[t]{.45\columnwidth}
        \includegraphics[width=1\textwidth]{fig/par_mu.png}
        \caption{ We keep $\mu_w = 10$, variate $\sigma^2_w$ and plot $r^2$ for different datasets.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.45\columnwidth}
        \includegraphics[width=1\textwidth]{fig/par_var.png}
        \caption{  We keep $\sigma^2_w$ = 1, variate $\mu_w$ and plot $r^2$ for different datasets. }
    \end{subfigure}
    \caption{ We plot how the parameters $(\mu_w, \sigma^2_w)$ affects the performance of ROVAE when noisy pairwise ordinal labels are observed. In this experiment, we randomly flipped $20\%$ of the labels (\ie $\eta = .2$). }
    \label{fig:my_label}
\end{figure}


\subsection{ Prior and Posterior Distribution for $s_{ij}$}
ROVAE introduces random variables $s_{ij}$ in the model. In this subsection, we first discuss how we choose parameters for the its prior distribution, parameterized by $\mu_w$ and $\sigma^2_w$; and how its aggregated posterior distribution $q(s_{ij}) = \frac{1}{|\mathcal{J}|}\sum_{(i, j) \in \mathcal{J}} q(s_{ij} | \mathbf{x}_i, \mathbf{x}_j )$ looks like at different noise levels. 



==> sections/intro_v1.tex <==
% !TEX root = ../main.tex

\section{Introduction}
\label{sec:introduction}
Disentanglement is a task of recovering the latent explanatory factors of variations in the data \citep{bengio2013representation}.
In recent years, several unsupervised disentanglement learning methods  \citep{higgins2017beta, kim2018disentangling, chen2018isolating, lopez2018information} have been proposed based on the variants of Variational Autoencoder (VAE). However, \citet{locatello2018challenging} demonstrate with theory and experiments that unsupervised disentanglement learning is fundamentally impossible if no inductive biases are provided. Therefore, methods with various forms of supervisions \cite{narayanaswamy2017learning,kulkarni2015deep, bouchacourt2018multi} have been propose to improve the performance for disentanglement. In this paper, we focus on discussing one specific supervision for disentanglement learning, where partial pairwise ordinal information is provided to learn one latent factor of interest. We propose a disentanglement method, we call Robust Ordinal VAE (ROVAE). Our proposed method incorporates pairwise ordinal labels in the VAE framework and is robust against noisy ordinal labels.

Traditionally, learning based on ordinal information can be separated into three categories~\citep{chen2009ranking}: pointwise
approach \citep{cossock2008statistical} that treats each single object as the learning instance; listwise approach \citep{cao2007learning} that views a provided ranked list of objects as the learning instance; and pairwise approach \citep{herbrich1999support, freund2003efficient, burges2005learning} that regards a pair of objects as the learning instance. Since it is straightforward to convert pointwise and listwise labels into pairwise labels, we focus on discussing the scenario where ordinal information is represented using pairwise labels. As far as we know, this is the first paper that utilizes pairwise ordinal labels in disentanglement learning.

This paper is motivated by a real-world problem of analyzing the severity of Chronic Obstructive Pulmonary Disease (COPD), which is a devastating disease related to cigarettes smoking. In clinical practice, the GOLD criteria \citep{singh2019global} is widely used to classify COPD patients into $5$ ordinal categories from healthy to very severe COPD, based on the severity of airflow limitation. Now that there are chest Computer Tomography (CT) images available, we want to investigate how CT images are related to disease severity. It is natural to use the GOLD criteria to guide the analysis for CT images during training. However, as demonstrated by \citet{matsuoka2010quantitative}, the CT appearance of the lungs can look similar in terms of severity, even in patients with very different levels of airflow limitations. This implies that the ordinal information (disease severity) represented using GOLD criteria is noisy for CT images. This motivates us to develop a model that is robust to noisy ordinal labels.

In this paper, we assume that in addition to the observations, we are also provided pairwise ordinal labels between instances, which represents whether or not one instance is greater than other instances, based on a specific factor of interest (\eg severity for the COPD). The goal is to learn the latent variable that represents this factor of interest. We proposed a disentangling model based on the VAE framework, incorporating the pairwise ordinal labels. Since the provided pairwise ordinal labels might be noisy, we introduce non-negative random variables to model the trustworthiness of each ordinal label. Introducing these random variables allows the proposed model to automatically determine whether a label is trustworthy, and learn the latent representation based on more trustworthy labels while ignoring less trustworthy labels. As shown in the empirical evaluations on several benchmark datasets and the real-world COPD dataset, the proposed method is able to better disentangle the factor of interest and it is more robust against noisy labels.

{\bf Contributions} \hspace{1mm}
The contributions of this paper are summarized as follows: (1)~We design a probabilistic model based on VAE framework, incorporating the pairwise ordinal labels. 
(2)~We introduce trustworthiness score in the model. This allows the model to automatically determine whether a label is trustworthy or not, and learn the latent representation based on more trustworthy labels while ignoring less trustworthy labels.
(3)~We conduct extensive experiments on benchmark datasets and the real-world COPD dataset. Experimental results demonstrate that the proposed method is more robust against noisy ordinal labels


==> sections/method_v1.tex <==
% !TEX root = ../main.tex


\section{Methods}

In the following sections, we first explain the general framework of ROVAE. We then discuss how we incorporate ordinal labels into the model and introduce how we model trustworthiness for each pairwise ordinal label. Finally, we summarize the overall model, and analyze the mechanism how trustworthiness score help improve robustness of ROVAE.


\subsection{General Framework}
\label{sec:method_framework}   
In this paper, we propose a probabilistic approach to model uncertainty, since we assmue both $\mathbf{X}$ and $\mathbf{Y}$ are noisy observations; 
We adopt the VAE framework \cite{kingma2013auto} such that $\mathbf{x}_n$ is reconstructed based on the latent variables $\mathbf{z}_{n}$.
We assume that for each instance $n$, the latent variable $\mathbf{z}_n$ is divided into two sub-spaces, {\it i.e., } $\mathbf{z}_n = [ u_n, \mathbf{v}_n ] $, where  $u_n \in \mathbb{R}$ represents the latent variable that corresponds to the factor of interest, while $\mathbf{v}_n \in \mathbb{R}^{D}$ accounts for the rest of information that is useful to reconstruct $\mathbf{x}_n$.  
Since $y_{ij}$ represents pairwise ordinal loss based on the factors of interest, it dependents on only the latent variable that corresponds to the factor of interest; {\it i.e., } $p(y_{ij} | \mathbf{z}_i , \mathbf{z}_j) = p(y_{ij} | u_i , u_j ) $. Therefore, the joint distribution of the observed instances and similarities has the following factorization,
\begin{equation}
\label{equ:decoder}
    \begin{adjustbox}{width=\columnwidth,center}
    {$
    p_{\boldsymbol{\theta}}(\mathbf{X}, \mathbf{Y}| \mathbf{U}, \mathbf{V}) = \prod_{n=1}^N p_{\boldsymbol{\theta}} ( \mathbf{x}_n | u_n, \mathbf{v}_n)
    \prod_{(i,j)\in \mathcal{J}} p(y_{ij} | u_i, u_j ).
    $}
    \end{adjustbox}
\end{equation}
In this equation,  $p_{\boldsymbol{\theta}}(\mathbf{x}_n |  u_n, \mathbf{v}_n )$ represents the reconstruction model of the VAE framework as shown in Section \ref{sec:background_VAE}. We explain $p(y_{ij} | u_i , u_j)$ in the next section.

\subsection{Incorporating Ordinal Loss}
\label{sec:method_ordinal}
One possible strategy to model $p(y_{ij} | u_i , u_j)$ is simply follow Equation (\ref{equ:logistic_y}), where we let $u_i = f(\mathbf{x}_i)$ and $u_j = f(\mathbf{x}_j)$. However, as mention in \ref{sec:related_work_ordinal}, this method does not consider the noise in the model. To solve this problem, we introduce a non-negative random variable $s_{ij}$, associated with each observed ordinal label $y_{ij}$. We call $s_{ij}$ trustworthiness score, such that a greater value of $s_{ij}$ indicates that $y_{ij}$ is more trustworthy and vice versa. With $s_{ij}$ introduced, we let
\begin{equation}
    \label{equ:y|s}
    \begin{aligned}
        p  (y_{ij} | u_i, u_j, s_{ij} ) = & 
        \left( \vphantom{\frac{1}{1}} \psi( s_{ij} (u_i - u_j) ) \right)^{y_{ij}}
        \\
        & \left( \vphantom{\frac{1}{1}} 1 - \psi( s_{ij} (u_i - u_j) ) \right)^{ 1 - y_{ij}},
    \end{aligned}
\end{equation}
where $\psi$ is the logistic function. Note that if $s_{ij} = 1$ for all $(i, j) \in \mathcal{J}$, then Equation (\ref{equ:y|s}) degenerate into Equation (\ref{equ:logistic_y}). If $s_{ij} \rightarrow 0$, we have $ p(y_{ij} = 1 | u_i, u_j, s_{ij} ) \approx 1/2$. If $s_{ij} \rightarrow \infty$, we have $ p(y_{ij} = 1 | u_i, u_j, s_{ij} ) \approx 1$ if $u_i > u_j$ and  $ p(y_{ij} = 0 | u_i, u_j, s_{ij} ) \approx 1$ if $u_i < u_j$. This allows the model to deal with the noisy ordinal labels that is discussed in Section \ref{sec:related_work_ordinal}. 


After defining the probability for $y_{ij}$ in Equation (\ref{equ:y|s}), the embedding results of $u_i$ and $u_j$ are affected more significantly, if a more trustworthy $y_{ij}$ is observed (\ie $s_{ij}$ is larger). At the same time, trustworthy score $s_{ij}$ are updated based on whether the label $y_{ij}$ is consistent with the current model during training. We analyze how this is achieved in Section \ref{sec:s_analysis}.

 


\subsection{Modelling Trustworthiness}
\label{sec:method_trustworthy}
Note that for a pair of real-valued random variables $t_i$ and $t_j$, it must satisfy the symmetric property that $p( t_i > t_j ) = 1 - p( t_i < t_j )$. Since $ y_{ij} $ is the indicator for the ordinal label as defined in Equation~(\ref{equ:y|s}), it requires $s_{ij} = s_{ji}$. Therefore, we introduce two real-valued auxiliary variables $w_{ij}$ and $w_{ji}$ that are i.i.d. samples from a normal distribution 
\begin{equation}
    w_{ij}, w_{ji} \sim \mathcal{N} (\mu_{w0}, \sigma_{w0}^2)
\end{equation}
and let $s_{ij} = ( w_{ij}^2 + w_{ji}^2) / 2$. We make this specific choice to make sure $s_{ij}$ both non-negative and symmetric. Letting $w_{ij}$ and $w_{ji}$ follow normal distribution also facilitates the optimization of the model, because we can make use of the reparameterization trick \citep{kingma2013auto}, where we can get samples of $s_{ij}$ by first sampling $w_{ij}$ and $w_{ji}$ from their approximated posterior distributions.

In our model, we want the mean value of $ s_{ij} $ to be large, because we do not want to ignore too many ordinal labels. We also want the variance of $s_{ij}$ to be relatively large such, which allows us to trust a subset of labels while ignore the others. We discuss how the choices of these parameters affect the performance of the model in details in Section \ref{sec:Experiments}.

In Section \ref{sec:method_framework} \ref{sec:method_ordinal} and \ref{sec:method_trustworthy}, we have introduced our decoder model $p_{\boldsymbol{\theta}}( \mathbf{X}, \mathbf{Y} | \mathbf{W}, \mathbf{Z})$. The model is summarized in Figure~\ref{fig:decoder}. 

\begin{figure}[t]
    \centering
    \begin{minipage}{.49\textwidth}
    \centering
    \begin{adjustbox}{max width= .7 \columnwidth}
        \input{fig/decoder.tex}
    \end{adjustbox}
    \caption{ The decoder model { \small $p_{\boldsymbol{\theta}}( \mathbf{X}, \mathbf{Y} | \mathbf{U}, \mathbf{V}, \mathbf{W})$}.}
    \label{fig:decoder}
    \end{minipage}
    \hfill
    \begin{minipage}{.49\textwidth}
    \centering
    \begin{adjustbox}{max width= .66 \columnwidth}
        \input{fig/encoder.tex}
    \end{adjustbox}
    \caption{ The encoder model { \small $q_{\boldsymbol{\phi}}(\mathbf{U}, \mathbf{V}, \mathbf{W}  | \mathbf{X})$ }.}
    \label{fig:encoder}
    \end{minipage}
\end{figure}

\subsection{ Approximating the Posterior Distribution }
After introducing our decoder model, we need to compute the posterior distribution for all random variables $p( \mathbf{Z}, \mathbf{W} | \mathbf{X}, \mathbf{Y})$. Since it is intractable to compute the posterior distribution in closed form, we use an encoder  $q_{\boldsymbol{\phi}}(\cdot| \cdot)$ to approximate it, such that it factorizes as
\begin{equation}
\begin{aligned}
    p( \mathbf{U}, \mathbf{V}, \mathbf{W} | \mathbf{X}, \mathbf{Y}) \approx 
    & \prod_{n=1}^N q_{\boldsymbol{\phi}}( u_n | \mathbf{x}_n )
    q_{\boldsymbol{\phi}}( \mathbf{v}_n | \mathbf{x}_n ) 
    \\
    & \prod_{(i, j) \in \mathcal{J}} q_{\boldsymbol{\phi}}( w_{ij} | \mathbf{x}_i, \mathbf{x}_j )
\end{aligned}
\end{equation}
where $\boldsymbol{\phi}$ is the parameters in the decoder. To facilitate the computation of gradient via reparameterization tricks \citep{kingma2013auto}, we let  $q_{\boldsymbol{\phi}} ( u_n | \mathbf{x}_n )$, $q_{\boldsymbol{\phi}} ( \mathbf{v}_n | \mathbf{x}_n )$ and $q_{\boldsymbol{\phi}} ( \mathbf{w}_{ij} | \mathbf{x}_i, \mathbf{x}_j )$ follow Gaussian distributions, which is consistent to the standard VAE framework. The decoder model is summarized in Figure~\ref{fig:encoder}. 

\subsection{Overall Model}
The overall objective function can be summarized as follows:
\begin{equation}
    \begin{aligned}
        \mathcal{L} = &
        \max_{ \boldsymbol{\phi}, \boldsymbol{\theta} }
        \mathbb{E}_{\mathbf{x}_n \sim \text{data} }
        [\mathbb{E}_{ q_{\boldsymbol{\phi}} ( \mathbf{z}_n | \mathbf{x}_n ) } 
        \log p_{\boldsymbol{\theta}} ( \mathbf{x}_n | \mathbf{z}_n ) ]
        \\
        & + \alpha \mathbb{E}_{ (i,j) \sim \mathcal{J} } 
        [\mathbb{E}_{ q_{\boldsymbol{\phi}}(u_i, u_j, w_{ij}| \mathbf{x}_i, \mathbf{x}_j)
        }
        [
        \log p( y_{ij} | u_i, u_j, w_{ij}
        ] ] 
        \\
        & - \beta \mathbb{E}_{\mathbf{x}_n \sim \text{data} }
         [ \mathcal{D}_{KL} ( q_{\phi}( \mathbf{z} ^{(u)}_n |\mathbf{x}_n) || \mathcal{N}( \boldsymbol{0}, \boldsymbol{I} ) ]
        \\
        & - \mathbb{E}_{ (i,j) \sim \mathcal{J} }
        [ \mathcal{D}_{KL} ( q_{\phi}( w_{ij} | \mathbf{x}_i, \mathbf{x}_j) || \mathcal{N}( \mu_w,  \sigma_w^2 ) ) ].
    \end{aligned}
    \label{equ:objective}
\end{equation}
The non-negative parameter $\alpha$ controls the trade off between the ordinal loss and other terms in the objective function. Similar to $\beta$-VAE \citep{higgins2017beta}, we introduce a parameter $\beta$ for the KL divergence term. As mensioned by \citet{mathieu2019disentangling}, introducing $\beta$ helps control the overlap of encodings in the latent space and therefore lead to better generalization of the latent representations. We solve the  optimization problem for $\boldsymbol{\theta}$ and $\boldsymbol{\phi}$ stochastic gradient descent (SGD). We discuss how the parameters $\alpha$ and $\beta$ impact the performance of the model in Section \ref{sec:Experiments}. 

\subsection{Analysis of Trustworthiness Score}
\label{sec:s_analysis}
After introducing the overall objective function, now we analyze how $u_i$, $u_j$ and $w_{ij}$ interact during training. In the $(t+1)$ iteration in the training, we consider the minibatch of pairwise labels $\mathcal{J}_{(t+1)}$. We first sample $u_i$, $u_j$, $s_{ij}$ for $(i,j) \in \mathcal{J}_{(t+1)}$ from the encoder model $q_{\boldsymbol{\phi}^{(t)}}$ via reparameterization trick, where $\boldsymbol{\phi}^{(t)}$ represents the current parameters for the encoder model. Now we analyze the second term in the objective function in Equation (\ref{equ:objective}), because it define how $u_i$, $u_j$ and $s_{ij}$ interact. By plugging Equation (\ref{equ:y|s}) into the second term  in Equation (\ref{equ:objective}), we have
\begin{equation}
    \begin{adjustbox}{width=\columnwidth,center}
    {$
    \begin{aligned}
    \label{equ:interaction}
        \mathcal{L}(u_i, u_j, s_{ij}) = & \alpha \frac{1}{|\mathcal{J}_{(t+1)}|}\sum_{(i,j) \in \mathcal{J}_{(t+1)}} y_{ij} \log \psi( s_{ij} (u_i - u_j) )
        \\
        & + (1 - y_{ij}) \log \psi( s_{ij} (u_j - u_i) )
    \end{aligned}
    $}
    \end{adjustbox}
\end{equation}

We first analyze how the embedding of $u_i$ and $u_j$ will be affected by the fixed $w_{ij}$ when we maximize this function with respect to $u_i$ and $u_j$. We observe in Equation (\ref{equ:interaction}) that if $y_{ij}$ is untrustworthy such that $s_{ij} \rightarrow 0$, since $\psi(0) = 1/2$ is a constant, $u_i$ and $u_j$ do not depend on $y_{ij}$. This indicates that when we embed $u_i$ and $u_j$ in the latent space, untrustworthy ordinal labels $y_{ij}$ will be ignored by the model. In contrast, if $s_{ij} >>0$, since the logistic function $\psi$ is monotonic increasing, $u_i - u_j$ tends to be large if $y_{ij} = 1$ and$u_j - u_i$ tends to be large if $y_{ij} = 0$, when we update $u_i$ and $u_j$. This implies that the trustworthy ordinal label $y_{ij}$ with large $s_{ij}$ will affect the embedding of $u_i$ and $u_j$ more significantly in the optimization.  

Now we analyze how $s_{ij}$ will be updated, assuming $u_i$ and $u_j$ are fixed, when we maximize Equation~(\ref{equ:interaction}). Because the logistic function $\psi$ is monotonic increasing, we observe that $s_{ij} \rightarrow \infty$ if ($y_{ij} = 1$ and $u_i > u_j$) or ($y_{ij} = 0$ and $u_i < u_j$); and $s_{ij} \rightarrow 0$, otherwise. Since $u_i$ and $u_j$ are sampled from the current encoder model $q_{\boldsymbol{\phi}^{(t)}}$ through the reparameterization trick, we conclude that $s_{ij}$ tend to have large value if $y_{ij}$ is consistent with the current encoder model $q_{\boldsymbol{\phi}^{(t)}}$ and vice versa.


==> sections/relatedWork_v1.tex <==
% !TEX root = ../main.tex

\section{ Related Work }
\subsection{Unsupervised Disentanglement with Variational Auto-Encoder (VAE)}
\label{sec:background_VAE}
There has been several unsupervised disentangling methods based on Variational Auto-Encoder (VAE) \citep{higgins2017beta, kim2018disentangling, chen2018isolating, lopez2018information}. In general, the objective function of these methods can be summarized as follows:
\begin{equation}
    \label{equ:obj_VAE}
    \begin{aligned}
    \mathcal{L}_{VAE} = & 
    \max_{\boldsymbol{\theta}, \boldsymbol{\phi}}
    \hspace{2mm}
    \mathbb{E}_{ \mathbf{x}_n \sim p_{\text{data}} } 
        [\mathbb{E}_{q_{\boldsymbol{\phi}}(\mathbf{z}_n|\mathbf{x}_n) }[\log p_{\boldsymbol{\theta}}(\mathbf{x}_n|\mathbf{z}_n)]
    \\
        & - \mathcal{D}_{KL} 
        \left( q_{\boldsymbol{\phi}}(\mathbf{z}_n|\mathbf{x}_n) || p(\mathbf{z})
        \right) - \beta \mathcal{R}( q_{\boldsymbol{\phi}}(\mathbf{z}_n|\mathbf{x}_n) 
        ]
    \end{aligned}    
\end{equation}
where $\mathbf{X} = \left\{ \mathbf{x}_n \right\}_{n =1}^{N}$ and $ \mathbf{Z} = \left\{ \mathbf{z}_n \right\}_{n =1}^{N}$ denote the observed samples and  the corresponding latent variables respectively, and $N$ is the number of samples. We use $ p_{\boldsymbol{\theta}}(\mathbf{x}_n|\mathbf{z}_n)$ and $q_{\boldsymbol{\phi}}(\mathbf{z}_n|\mathbf{x}_n)$ to represent the decoder and encoder networks that are parameters by $\boldsymbol{\theta}$ and $\boldsymbol{\phi}$, respectively. We let $\mathcal{D}_{KL}(\cdot || \cdot)$ denote the KL divergence and $p(\mathbf{z})$ denote prior distribution for $\mathbf{z}$. In this paper, we let $p(\mathbf{z})$ be an isotropic unit Gaussian distribution. $ \mathcal{R}(\mathbf{Z}) $ is a regularization term that forces each dimension of $\mathbf{Z}$ to be independent with each other. $\beta$ is a non-negative hyper-parameter that controls the weight of $ \mathcal{R}(\mathbf{Z}) $. 

Existing unsupervised disentangling methods chooses different $ \mathcal{R}(\mathbf{Z}) $. $\beta$-VAE \citep{higgins2017beta} let $ \mathcal{R}(\mathbf{Z}) = \mathcal{D}_{KL} \left( q_{\boldsymbol{\phi}}(\mathbf{z}_n|\mathbf{x}_n) || p(\mathbf{z}) \right)$. Both factor-VAE \citep{kim2018disentangling} and $\beta$-TCVAE \citep{chen2018isolating} let $ \mathcal{R}(\mathbf{Z}) $ be approximations of the total correlation of $\mathbf{Z}$, where factor-VAE approximates it with an adversarial loss and $\beta$-TCVAE approximates it using its lower bound. HCV \citep{lopez2018information} defines $\mathcal{R}(\mathbf{Z})$ based on Hilbert-Schmidt Independence Criterion (HISC) \citep{10.1007/11564089_7}. However, without explicit supervision, it is difficult to control the correspondence between a learned latent variable and a semantic meaning, and it is not guaranteed that the factor of interest can always be successfully disentangled \cite{locatello2018challenging}. In contrast, our proposed method utilizes the pairwise ordinal labels as explicit supervision, which encourages the model to disentangle the factor of interest.

\subsection{Supervised Disentanglement Methods}

There have been attempts to improve disentanglement performance by introducing supervision of various forms.
\citet{narayanaswamy2017learning} and \citet{kulkarni2015deep} propose semi-supervised VAE methods that learn disentangled representation, by making use of partially observed class labels or real-value targets. \citet{bouchacourt2018multi} introduces supervision via grouping the samples. \citet{feng2018dual, chen2018multiview, chen2019weakly} propose to make use of pairwise similarity labels. In contrast, our proposed method utilizes pairwise ordinal labels as the supervision.

\subsection{Pairwise Ordinal Losses}
\label{sec:related_work_ordinal}
Many existing methods make use of the ordinal information with different motivations and formulations. In general, these methods can be divided into three categories \citep{chen2009ranking}: The pointwise approach \citep{cossock2008statistical, li2008mcrank}, which considers each single instance independantly in the objective function; the pairwise approach \citep{herbrich1999support, freund2003efficient, burges2005learning}, which analyzes a pair of instances at a time in the loss function; and the listwise approach \citep{cao2007learning, xia2008listwise}, which considers entire list of instances simutaneously. 

In this paper, we focus on discussing pairwise ordinal loss, where the partial order are provided using a set of pairwise ordinal labels, denoted by $ \mathbf{Y} = \{ y_{ij} \}_{ (i,j) \in \mathcal{J} }$, We let $\mathcal{J}$ represent the partially observed set of pairwise orders, \ie $\mathcal{J} \subseteq \{ (i,j)| i, j \in \{ 1, \ldots ,N \} \}$. We ;et $y_{ij}$ be binary ($y_{ij} \in \{ 0,1\}$) , where $y_{ij} = 1$ indicates  the latent factor of variations satisfying $t_i > t_j$ and vice versa. The existing methods model the ordinal loss with hinge function~\citep{herbrich1999support}, exponential function~\citep{freund2003efficient} and logistic function~\citep{burges2005learning}, respectively. In this paper, since we focus on developing a probabilistic model, we focus on discussing the logistic function case, where $y_{ij}$ is modeled as a random variable such that
\begin{equation}
    \label{equ:logistic_y}
    \begin{aligned}
    p  (y_{ij} | \mathbf{x}_i, \mathbf{x}_j ) = &
        \left( \vphantom{\frac{1}{1}} \psi(f(\mathbf{x}_i) - f(\mathbf{x}_j) ) \right)^{y_{ij}}
    \\
        & \left( \vphantom{\frac{1}{1}} 1 - \psi(f(\mathbf{x}_i) - f(\mathbf{x}_j) ) \right)^{ 1 - y_{ij}},
    \end{aligned}
\end{equation}
where $\psi$ is the logistic function, \ie $\psi(t) = 1 / (1 + e^{-t})$, and $f(\mathbf{x})$ is a certain function that captures the ordinal information for instance $\mathbf{x}$. 

Note that in Equation (\ref{equ:logistic_y}), if $f(\mathbf{x}_i) \approx f(\mathbf{x}_j)$, then it is always true that $p  (y_{ij} = 1 | \mathbf{x}_i, \mathbf{x}_j ) \approx 1 / 2$. However, as discussed in Section \ref{sec:introduction}, the pairwise ordinal labels might be noisy in COPD dataset, because the CT images might look similar (\ie $f(\mathbf{x}_i) \approx f(\mathbf{x}_j)$), but the airflow limitations might differ significantly(\ie either $p  (y_{ij} = 0| \mathbf{x}_i, \mathbf{x}_j ) \approx 1$, or $p  (y_{ij} = 1| \mathbf{x}_i, \mathbf{x}_j ) \approx 1$). Therefore, using Equation (\ref{equ:logistic_y}) might not be sufficient for analyzing noisy ordinal labels. To solve this problem, we introduce a random variable, we call trustworthiness score, associated with each pairwise ordinal label. with the trustworthiness score introduced, our model is more robust against noisy ordinal labels. 


